Rapid quantitative chemical composition mapping using model-based MRI reconstruction with field inhomogeneity correction

Magnetic resonance spectroscopic imaging methods are particularly attractive for chemical engineering applications, including the monitoring of chemical reactions, where a rapid assessment of spatial variations in chemical composition is required. Conventional approaches, such as chemical shift imaging, introduce an additional spectral-encoding dimension, which substantially increases acquisition time. Consequently, fast spatially resolved spectroscopy remains an active research topic. This work uses a model-based reconstruction framework that embeds a priori spectral knowledge of the involved chemical components into the forward model to accelerate composition mapping. It allows for the reconstruction of molar ratio maps for individual chemical components without acquiring high-resolution spectra. Extending from previous studies, the proposed model accounts for inhomogeneities of the main field, which become more pronounced in systems with larger bores relevant for process engineering. Phantom experiments employing a 2D multi-gradient echo sequence demonstrate the ability to determine molar ratios for chemical components with single peaks as well as multiple peaks in their spectra. The bias and precision of the method remain around 0.01 mol/mol and 0.09 mol/mol, respectively, for a 20 s scan, indicating suitability for dynamic processes. Finally, acquisition time can be reduced further by applying sparse k-space sampling, potentially shortening the scan to 5 s with only minor degradation in quantitative performance.

==> math-definitions.tex <==
% Math definitions
\usepackage{nicefrac}

\usepackage{bbm}
\newcommand{\IN}{\mathbb{N}}		% natural   numbers
\newcommand{\IZ}{\mathbb{Z}}		% integers
\newcommand{\IQ}{\mathbb{Q}}		% rational  numbers
\newcommand{\IR}{\mathbb{R}}		% real      numbers
\newcommand{\IC}{\mathbb{C}}		% complex   numbers
\newcommand{\IS}{\mathbb{S}}		% sphere
\newcommand{\cB}{\mathcal{B}}       % ball

\renewcommand{\epsilon}{\varepsilon}				% nicer Epsilon
% \renewcommand{\theta}{\vartheta}                  	% nicer Theta
\renewcommand{\phi}{\varphi}						% nicer Phi

\newcommand{\set}[1]{\left\{ #1 \right\}}				% set
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}		% absolute value
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}		% norm
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}	% floor
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}		% ceiling
\newcommand{\onot}[1]{\mathcal{O}{\left( #1 \right)}}	% Big O notation

\newcommand{\signatur}[3]{#1:#2\,\rightarrow\,#3}     %function signature


% definitions
\newcommand{\DF}{\textup{DF}}
\newcommand{\SF}{\textup{SF}}
\newcommand{\signal}{\textup{Signal}}
\newcommand{\Reco}{\textup{Reco}}
\newcommand{\bxi}{ {\boldsymbol\xi} }
\newcommand{\bnu}{ {\boldsymbol\nu} }
\newcommand{\bla}{ {\boldsymbol\lambda} }
\newcommand{\brho}{ {\boldsymbol\rho} }
\newcommand{\bsi}{ {\boldsymbol\sigma} }

\newcommand{\zb}[1]{\mbox{\boldmath{${#1}$}}}
\newcommand{\zbs}[1]{\mbox{\boldmath\scriptsize{${#1}$}}}
\newcommand{\zbss}[1]{\mbox{\boldmath\tiny{${#1}$}}}
\renewcommand{\d}{\, \text{d}}
\newcommand{\adj}{{\vdash \hspace*{-1.752mm} \dashv}}
\newcommand{\one}{\mbox{\boldmath{$1$}}}

% siunitx setup
\usepackage[binary-units = true,exponent-product = \cdot]{siunitx}
\sisetup{list-final-separator = {, and },  % use final comma in SIlist
		list-units = single,
        range-units = single,
        product-units = power,
        separate-uncertainty, % align +- in a table
        %table-align-uncertainty=true, % ändert nichts
        }
% New SI constant
\DeclareSIUnit{\vacuumpermeability}{\text{$\mu_0$}}

% PGFPlots setup (colormap inferno)
\pgfplotsset{
colormap/inferno/.style={%
    /pgfplots/colormap={inferno}{%
      rgb=(0.001462, 0.000466, 0.013866)
      rgb=(0.037668, 0.025921, 0.132232)
      rgb=(0.116656, 0.047574, 0.272321)
      rgb=(0.217949, 0.036615, 0.383522)
      rgb=(0.316282, 0.053490, 0.425116)
      rgb=(0.410113, 0.087896, 0.433098)
      rgb=(0.503493, 0.121575, 0.423356)
      rgb=(0.596940, 0.154848, 0.398125)
      rgb=(0.688653, 0.192239, 0.357603)
      rgb=(0.775059, 0.239667, 0.303526)
      rgb=(0.851384, 0.302260, 0.239636)
      rgb=(0.912966, 0.381636, 0.169755)
      rgb=(0.956852, 0.475356, 0.094695)
      rgb=(0.981895, 0.579392, 0.026250)
      rgb=(0.987464, 0.690366, 0.079990)
      rgb=(0.973088, 0.805409, 0.216877)
      rgb=(0.947594, 0.917399, 0.410665)
      rgb=(0.988362, 0.998364, 0.644924)
    },
  },}

%% Colors
\definecolor{ibilight}{RGB}{193,216,237}
\definecolor{ibidark}{cmyk}{1.00,0.69,0.00,0.12}
\definecolor{uke2}{cmyk}{0.10,0.18,0.25,0.36}
\definecolor{uke3}{cmyk}{0.00,0.00,0.00,0.80}
\definecolor{ukesec1}{cmyk}{0.00,0.09,1.00,0.00}
\definecolor{ukesec2}{cmyk}{0.00,0.61,0.99,0.00}
\definecolor{ukesec3}{cmyk}{0.59,0.00,0.22,0.00}
\definecolor{ukesec4}{cmyk}{0.54,0.00,1.00,0.00}
\definecolor{tuhh}{cmyk}{0.65,0.00,0.20,0.00}

